Securing Federated Learning against Backdoor Threats with Foundation Model Integration

Federated Learning (FL) enables decentralized model training while preserving privacy. Recently, the integration of Foundation Models (FMs) into FL has enhanced performance but introduced a novel backdoor attack mechanism. Attackers can exploit FM vulnerabilities to embed backdoors into synthetic data generated by FMs. During global model fusion, these backdoors are transferred to the global model through compromised synthetic data, subsequently infecting all client models. Existing FL backdoor defenses are ineffective against this novel attack due to its fundamentally different mechanism compared to classic ones. In this work, we propose a novel data-free defense strategy that addresses both classic and novel backdoor attacks in FL. The shared attack pattern lies in the abnormal activations within the hidden feature space during model aggregation. Hence, we propose to constrain internal activations to remain within reasonable ranges, effectively mitigating attacks while preserving model functionality. The activation constraints are optimized using synthetic data alongside FL training. Extensive experiments demonstrate its effectiveness against both novel and classic backdoor attacks, outperforming existing defenses.

==> sec/responses.tex <==
\section*{Author Responses}

\subsection{Response to Reviewer \#8}
We believe Reviewer \#8's assessment may stem from a \textit{\textbf{lack of familiarity with the field}}, as their comments \textit{\textbf{contradict those of other reviewers}}. Additionally, \textit{\textbf{many of their concerns are already clearly addressed in our paper}}. Below, we provide our responses to their major points.

\noindent\textbf{(a) Importance/relevance to ICME}
Reviewer \#8 questions our work's relevance to ICME, claiming limited interest and a lack of multimedia elements.
However, \textit{this contradicts the opinions of other 3 reviewers}, who found our work sufficiently relevant to ICME.
Besides, as stated in Sec.~\ref{sec:method}, our proposed method is modality-agnostic. In Sec.~\ref{sec:exp}, we evaluate its effectiveness using widely accepted machine learning benchmarks.

\noindent\textbf{(b) Novelty/originality}
Reviewer \#8 claims our method lacks novelty because existing methods can address the vulnerability in FM-FL, but this overlooks our key contributions.
As detailed in Sec.~\ref{sec:method} and Sec.~\ref{sec:exp}, applying existing defenses to federated learning with foundation models (FL-FM) presents \textbf{significant challenges that our approach addresses}:
\textbf{(b.1) Data Availability}: Existing defenses require \textit{clean real data} for threshold selection and maintain model performance, which is infeasible in our scenario with \textit{only poisoned synthetic data}. We address this with a dynamic trade-off mechanism for accuracy and mitigation (Eq.~\ref{eq:opt_func}).
\textbf{(b.2) Application to FL}: Unlike centralized ML, FL involves decentralized training, multiple communication rounds, and heterogeneous client models, making defense strategies more complex. Our method is specifically designed to handle these challenges.
\textbf{(b.3) Efficiency}: FL is an ongoing process, requiring defenses to be applied in every round. We optimize our strategy by selecting key layers and reducing iterations (See algorithm ~\ref{alg:defense} and ``Defense settings'' in Sec~\ref{sec:exp_setup}, ensuring both scalability and effectiveness.

\noindent\textbf{(c) Experimental validation and reproducibility}
Reviewer \#8 claims our paper lacks details on the experimental setup, but \textbf{Sec. ~\ref{sec:exp_setup} explicitly provides them}: datasets and model architectures in ``Datasets and Models,'' and hyperparameter configurations in ``Training Settings.''

The reviewer also vaguely suggests improvements for robustness without specifying any aspects. This assertion \textbf{lacks concrete reasoning and contradicts the assessments of other reviewers}, who acknowledge that our experiments thorough and valid.

\subsection{Response to Reviewer \#9}
Thank you for your positive feedback. We acknowledge your suggestion regarding exploring more robust optimization methods beyond synthetic datasets, and we will consider this in our future work.

\subsection{Response to Reviewer \#10}

We believe Reviewer \#10's assessment results from \textbf{negligence in paper reading and the resulting misunderstanding} rather than an actual issue with our work.
Their major concern -- that the attack success rate (ASR) has not decreased enough -- stems from a misinterpretation of the metrics used in our paper.
However, \textbf{our presentation is sufficiently clear}, as the other 3 reviewers correctly understood the ASR results.

\noindent\textbf{(a) Novelty/originality}
First, the reviewer’s reasoning does \textbf{not directly relate to originality} -- one concerns clarity, while the other relates to experimental validation.

Besides, both claims are unfounded:
\textbf{(a.1)} The reviewer questions why our defense is a separate stage rather than part of Stage 3. Stage 3 optimizes global model parameters, while Stage 4 optimizes defense parameters -- \textit{two distinct sets of parameters.} 
Separating them ensures clarity and modularity. 
Besides, Stage 3 is established in prior work, we focus on Stage 4 to avoid redundancy and due to space constraints.
\textbf{(a.2)} The reviewer misinterprets our results, stating that ``the ASR is minimally decreased (no more than 10\%).'' 
However, as shown in Section ~\ref{sec:exp}, we report the final ASR after defense, not just the reduction percentage -- our method reduces ASR to 10\%, not by 10\%. 
\textbf{This distinction is clearly presented, and no other reviewers raised similar concerns.}

% Our results demonstrate the effectiveness of the proposed method across diverse settings, as also acknowledged by Reviewers \#9 and \#11.

\noindent\textbf{(b) Technical correctness}
The reviewer's concerns arise from misunderstandings, which, once clarified, indicate no technical errors.
\textbf{(b.1)} These statements describe different aspects of the system and are \textbf{not contradictory}.
The server queries the FM to generate synthesized data that mirrors real local data as it knows the data category. 
The attacker, based on the FM application scenario, manipulates the server's queries to manipulate the synthesized data at the server.
This aligns with prior work and is not the focus of our paper not the focus of our paper-- we adopt an existing framework to study its vulnerabilities and propose a solution. 
The reviewer’s concern appears to stem from \textbf{unfamiliarity} with the field’s background, rather than an issue with our presentation.

\textbf{(b.2)} This misrepresents our explicitly defined threat model in Section ~\ref{sec:method}.
\textbf{We never assume that the server itself is adversarial.}
attackers exploit the server’s FM queries to inject backdoor instructions, but the server itself is not the attacker. This follows standard threat models (e.g., \cite{BD_ICL}), and there is no scenario where both the attacker and defender exist on the server side.
To further enhance clarity, we will provide an example attack scenario in the paper. However, the concerns raised by the reviewer do \textbf{not indicate a technical flaw but rather a misunderstanding of our definitions}.

\noindent\textbf{(c) Experimental validation and reproducibility}
% The reviewer acknowledges that we conducted experiments across different attacks and datasets but claims that our contributions are unconvincing due to a ``minimal decrease'' in ASR.
This concern arises again from a misinterpretation of our results, as already addressed in (a) Novelty and Originality. 
% The reviewer overlooks that we report the final ASR after applying our defense, rather than just the reduction percentage.
This misunderstanding appears to stem from the reviewer’s \textbf{negligence in carefully reading the paper}, as no other reviewers raised similar concerns.

\subsection{Response to Reviewer \#11}
Thank you for your constructive and positive feedback.
We acknowledge your suggestions regarding deeper theoretical analyses, ablation studies, sensitivity analyses, and efficiency evaluations. Due to page limits, we included only the primary experimental results. We will address your recommendations in the final paper version and future work.

